Image edge enhancement for effective image classification

Image classification has been a popular task due to its feasibility in real-world applications. Training neural networks by feeding them RGB images has demonstrated success over it. Nevertheless, improving the classification accuracy and computational efficiency of this process continues to present challenges that researchers are actively addressing. A widely popular embraced method to improve the classification performance of neural networks is to incorporate data augmentations during the training process. Data augmentations are simple transformations that create slightly modified versions of the training data and can be very effective in training neural networks to mitigate overfitting and improve their accuracy performance. In this study, we draw inspiration from high-boost image filtering and propose an edge enhancement-based method as means to enhance both accuracy and training speed of neural networks. Specifically, our approach involves extracting high frequency features, such as edges, from images within the available dataset and fusing them with the original images, to generate new, enriched images. Our comprehensive experiments, conducted on two distinct datasets CIFAR10 and CALTECH101, and three different network architectures ResNet-18, LeNet-5 and CNN-9 demonstrates the effectiveness of our proposed method.

==> tex/method-1.tex <==
\section{\uppercase{methodology}}
\subsection{Problem definition}

Let us define a labelled data set $ D\ =\ (x_i,y_i)$, where $x_i $ represents the $i^{th}$  image and $y_i$ represents the corresponding class label.  The data set contains labelled images each with three given channel (the RGB channels), the data set will be further split into three sections: training set, ${D_{\train}=\ ({x}_i,y_i})$, validation set,  $ {D_{\val}=\ ({x}_i,y_i})$ and testing set, ${D_{\test}=\ ({x}_i,y_i}).$ We use $D_{\train}$ to train a neural network, that consists of a backbone $f_{\theta}$ and a classifier $g_{\phi}$. The validation set $D_{\val}$ is used in order to save the model with the highest validation accuracy. Finally, we use $D_{\test}\ $ to calculate the test set classification accuracy. 

\subsection{Feature extraction}


We extract the edges of every image in $D_{\train}$ using the canny edge detector, \alert{the sigma $\sigma$ of the Gaussian filter in our experiment is fixed at a value of 3.} \mich{this info should be included in the experiments section.}


\subsection{Edge enhancement}
\alert{The idea of edge enhancement is to transform the training set $D_t$ labelled images to their edge enhanced version, turning the original training data set to $\ {\widetilde{D}}_t=\ {{\widetilde{x}}_i^t,{\widetilde{y}}_i^t}$} \mich{this is a bit convoluted, in method we focus on describing what the method does not motivation}, the transformed image set has the same size as the original training data set. The edge enhancement image pre-processing can be demonstrated as shown in \autoref{fig:example1}, where the leftmost labelled image is the original data, after canny filtering the extracted edges are shown and the rightmost labelled image is the edge enhanced result.  \alert{We first apply normalization to the sample images, and then resize the images based on the data sets to ensure the size is constant and suitable for the selected  convolution neural networks (CNN) and residual neural networks (ResNet)} \mich{is all this really needed here? } \cite{he2015spatial},\cite{hussain2020iot}. Canny filters are then applied to the data at each of its  RGB channels, the extracted edge information are merged with their original version to obtain the transformed image set, each with their labels corresponding to the original classes. 

%----------------------------------------------------------------------------------------
\begin{figure*}[h]
  \centering
\includegraphics[width=\textwidth, height = 0.22\textwidth]{fig/edge_enhancement.pdf}  
\caption{The flowchart of the edge enhancement method for model training. i) Original labelled data (batch size of 4) is edge enhanced to the transformed labelled data. ii) The original and transformed labelled data is concatenated as a batch of size 8, then feed into the network. iii) Model training. iv) Classification results obtained through test data set.}
  \label{fig:example1}
 \end{figure*}
%-------------------------------------------------------------------------------------------

\subsection{Training phase}

\alert{The batch size under consideration is 4} \mich{more appropriate to be written in the experiments section}, meaning that during each batch, \alert{edge enhancement is applied to a set of four training set images at a time} \mich{implementation details}, as shown in \autoref{fig:batch4}, where the top four images are the original data, the bottom four belongs to the edge enhanced data set. The edge enhanced images will be concatenated with the original training set images to form the inputs to the network model,as a total of 8 images during each batch sample to generate classification results. The corresponding algorithm pseudo codes are demonstrated in algorithm 1, and corresponding flow chart is shown in figure 3.


During the forward propagation, We extract the features $\vv_i$ by inputting every labelled image $\vx_i$ into the canny edge detection function $Canny()$, they can be expressed as  
\begin{equation}
    \vv_i \defn Canny(x_i)
\end{equation}
The extracted feature $\vv_i$ is then added with the original input $\vx_i$  to form the edge enhanced and labelled image $\vE_i$ . 
\alert{Let us define the network backbone as $M()$, and the vectors contain four (batch size)} \mich{definitions of networks and everything we should be in the problem definitions} original data and the edge enhanced data as $T_{x_i}$,$T_{v_i} $ with corresponding class label vector $T_{y_i} $ \mich{define this in problem definition}. During training phase, the data vectors will be concatenated to form the input data set $Im = \{{T_{x_i},T_{v_i}}\}$, and the corresponding concatenated class set $Lab = \{{T_{y_i},T_{y_i}}\}$ . The model output $O_{M} $  can then be presented as 

\begin{equation}
    \vO_{M} \defn M(Im,Lab)
\end{equation}
We pass $O_{M} $ to $C_{linear}$ \mich{define in problem definitions} which is the classifier (last layer of the network) so that \mich{in the equation below i see different symbols, unify them i think rename $O_M$ to $v_i$ for image i}

\begin{equation}
    \vz_i \defn C_{linear}(\vv_i)
\label{eq:logits}
\end{equation}
where $\vz_i$ is the vector of logits of image $i$. We obtain the probability of each class $\hat{p_i}$ by using the softmax activation function

\begin{equation}
    \hat{p_i} \defn \frac{\exp(\vz_i))}{\sum_{i=1}^N \exp(\vz_{i})},
\label{eq:softmax}
\end{equation}
where $N$ is the total number of classes. \alert{The loss function used in this experiment is the cross entropy loss function due to its great performance under multi-class classification tasks\cite{zhou2019mpce}.} With the aid of equation \eq{softmax}, we calculate the cross-entropy loss 
\begin{equation}
   L_{ce} \defn -\displaystyle \sum_{i \in N}\hat{q_i}\log(\hat{p_i}),
\label{eq:ce}
\end{equation}
Where $\hat{q_i}$ represents the true class probability. Back propagation is then performed to calculate the gradient of $L_{ce}$ with respect to the network weight \mich{use definition of your network}. For our choice of optimizer for network weight update, \alert{we use Stochastic Gradient Descent (SGD) with a momentum of 0.9, weight decay of 0.0005,  and  learning rate of 0.01.} 
\section{Inference}
Finally, forevery ima
, i ∈ [M],
we predict the pseudo-label
\begin{equation}
    \vY_i \defn argmax(\hat{p_i})
\end{equation}
$\vY_i$ is compared with the true labels $y_i^{Tr}$ to generate the overall classification accuracy,  
\begin{equation}
    \vS_c \defn Acc(\vY_i,y_i^{Tr})
\end{equation}
Where $\vS_c$is the overall classification accuracy, and $Acc$ is the accuracy function that sums every comparison results between the prediction and true class labels, the result is also divided by the total label size and multiplied by a hundred to be scaled to percentage.   \BlankLine
 




\begin{algorithm}[!h]
 \caption{Edge enhancement procedure}
 \SetKwInOut{Input}{input}
 \SetKwInOut{Output}{output}
 \Input{training data set ${D_t=\ {x}_i^t,y_i^t}$}
\Input{edge enhanced data set ${\widetilde{D}}_t=\ {{\widetilde{x}}_i^t,{\widetilde{y}}_i^t}$}
\Output{trained neural network model}
 
  batch size: 4;
  \BlankLine
\If{$D_t\ \in\ \ $ CALTECH101}
 {\State  $D_t\ $= Resize($D_t$, 256 x 256), 
 \BlankLine$D_t\ $= CenterCrop($D_t$, 224 x 224)  }
 \BlankLine
 $D_t$ = Normalization($D_t$)
 \BlankLine
 \While{epoch not finished}
 { \For{ i <= $D_t$.size() }{
  {\BlankLine feature = Canny($x_i^t$,sigma = 3),\BlankLine
  ${ \widetilde{x}}_i^t $ = add($x_i^t$,feature),
   \BlankLine Inputs = concat($x_i^t$ ${\widetilde{x}}_i^t$) 
}
 }
 \BlankLine
  Model = Model.train(Inputs, D_v)
 }

\end{algorithm}




